Bayesian Multi-Scale Optimistic Optimization

Bayesian optimization is a powerful global optimization technique for expensive black-box functions. One of its shortcomings is that it requires auxiliary optimization of an acquisition function at each iteration. This auxiliary optimization can be costly and very hard to carry out in practice. Moreover, it creates serious theoretical concerns, as most of the convergence results assume that the exact optimum of the acquisition function can be found. In this paper, we introduce a new technique for efficient global optimization that combines Gaussian process confidence bounds and treed simultaneous optimistic optimization to eliminate the need for auxiliary optimization of acquisition functions. The experiments with global optimization benchmarks and a novel application to automatic information extraction demonstrate that the resulting technique is more efficient than the two approaches from which it draws inspiration. Unlike most theoretical analyses of Bayesian optimization with Gaussian processes, our finite-time convergence rate proofs do not require exact optimization of an acquisition function. That is, our approach eliminates the unsatisfactory assumption that a difficult, potentially NP-hard, problem has to be solved in order to obtain vanishing regret rates.

==> background.tex <==



==> cumulative_regret.tex <==
\subsubsection{Cumulative Regret}

% Let $\hat{c}_1 = \left[2BQ \frac{C}{c_1^2} + 2\right]\frac{1}{\gamma}$,
$\hat{c}_2 = \left[2 + \frac{4BQ}{ c_2 \gamma} + \frac{2c_1}{c_2\gamma}\right]$.
% 
% \begin{mydefinition}
%  Let $\hat{I_h} = \{ (h, i) : f(\vx_{h, i}) + \hat{c}_{\alpha} \delta(h) \geq f^* \}$
% \end{mydefinition}

\begin{lemma}
 \label{levelvar}
 If any node $\vx_{h, i}$ or one of its descendants is evaluated, 
 then $\sup_{\vx \in \calX_{h, i}} \sigma(\vx) 
 \leq Q\left(\frac{\delta(h)}{c_1}\right)^{2/{\alpha}}$.
\end{lemma}
\begin{proof}
 Since $\sup_{\vx \in \calX_{h, i}} c_1\|\vx_{h, i}-\vx\|^{\alpha}
 \leq \delta(h) $, 
 we have $\sup_{\vx \in \calX_{h, i}} \|\vx_{h, i}-\vx\|
 \leq \left(\frac{\delta(h)}{c_1}\right)^{1/{\alpha}} $.
 Thus for any two $\vx_1, \vx_2 \in \calX_{h, i}$, 
 $\|\vx_1 - \vx_2\|^2 \leq 4\left(\frac{\delta(h)}{c_1}\right)^{2/{\alpha}}$.
 By Lemma~\ref{}, we have the statement.
\end{proof}



% \begin{lemma}
%  \label{alaph1}
%  If $\vx^*_{h}$ is reached and every node $\vx$ at level $h$ 
%  with $\vx \in \hat{I}_h$
%  has been evaluated,
%  then every node that is 
%  $\hat{c}_1\delta(h+1)$-suboptimal together with all
%  its descendants would not be evaluated again.
% \end{lemma}
% \begin{proof}
%  If every node $\vx$ on level $h$ is evaluated then by Lemma~\ref{levelvar}
%  $\sigma(\vx) < Q \left(\frac{C }{c_1}\right)^2 \gamma^{2h}$ $\forall \vx$. 
%  If a node $\vx$ were to be evaluated, it must be that 
%  $f(\vx) + 2B\sigma(\vx) \geq f^+$. Since $\vx^*_{h}$ is reached, 
%  $f^+ > f^* - \delta(h)$.
%  Thus $f(\vx) + 2B\sigma(\vx) \geq f^* - \delta(h)$ which implies that 
%  $$f^* - f(\vx) \leq 2B\sigma(\vx) + \delta(h) 
%  \leq \left[2BQ\left(\frac{C }{c_1}\right)^2 + C\right]\gamma^h$$
%  since $\gamma^{2h} \leq \gamma^h$. If $f^* - f(\vx_{h+1, i}) > 
%  \left[2BQ\left(\frac{C}{c_1}\right)^2 + C\right]\gamma^h + C\gamma^h 
%  = \hat{c}_1\delta(h+1)$, 
%  the by Lipschitz continuity, any descendant $\vx$ of $\vx_{h+1, i}$ would
%  be such that $f^* - f(\vx) > 
%  \left[2BQ\left(\frac{C}{c_1}\right)^2 + C\right]\gamma^h$.
%  Thus every node that is $\hat{c}_1 \delta(h+1)$-suboptimal is not in the 
%  ball thus together with its descendants would never be evaluated again.
% \end{proof}
% 
% \begin{lemma}
%  \label{alaph2}
%  If $\vx^*_{h}$ is reached and every node $\vx$ at level $h$ 
%  with $\vx \in \hat{I}_h$
%  has been evaluated,
%  then every node at level $h+1$ that is 
%  $\hat{c}_2\delta(h+1)$-suboptimal together with all
%  its descendants would not be evaluated again.
% \end{lemma}
% \begin{proof}
%  If every node $\vx$ on level $h$ is evaluated then by Lemma~\ref{levelvar}
%  $\sigma(\vx) < \frac{QC}{c_1} \gamma^h$ $\forall \vx$. 
%  If a node $\vx$ were to be evaluated, it must be that 
%  $f(\vx) + 2B\sigma(\vx) \geq f^+$. Since $\vx^*_{h}$ is reached, 
%  $f^+ > f^* - \delta(h)$. Thus 
%  $f(\vx) + 2B\sigma(\vx) \geq f^* - \delta(h)$ which implies that 
%  $$f^* - f(\vx) \leq 2B\sigma(\vx) + \delta(h) 
%  \leq \left[\frac{2BQC}{c_1} + C\right]\gamma^h.$$
%  Also $c_2\|\vx - \vx^*\|^2 \leq f^* - f(\vx) \leq 2B\sigma(\vx) + \delta(h) 
%  \leq \left[\frac{2BQC}{c_1} + C\right]\gamma^h$. Thus 
%  $\vx \in \calB\left(\vx^*, \sqrt{\left[\frac{2BQC}{c_1 c_2} 
%  + \frac{C}{c_2}\right]\gamma^h}\right).$
%  As the radius of a node on level $h+1$ is less than 
%  $\sqrt{\frac{C}{c_1}\gamma^{h+1}}$, if 
%  $\vx \notin \calB\left(\vx^*, \sqrt{\frac{C}{c_1}\gamma^{h+1}} + 
%  \sqrt{\left[\frac{2BQC}{c_1 c_2} + \frac{C}{c_2}\right]\gamma^h}\right)$
%  for $\vx$ on level $h+1$,
%  then none of its descendants would be evaluated again.
%  Now notice that for every node  
%  $\vx \in \calB\left(\vx^*,  \left(\sqrt{\frac{C}{c_1}\gamma^{h+1}} + 
%  \sqrt{\left[\frac{2BQC}{c_1 c_2} + \frac{C}{c_2}\right]\gamma^h}\right)\right)$, 
%  \begin{eqnarray*}
%   f^* - f(\vx) &\leq& c_1 \left(\sqrt{\frac{C}{c_1}\gamma^{h+1}} + 
%   \sqrt{\left[\frac{2BQC}{c_1 c_2} + \frac{C}{c_2}\right]\gamma^h}\right)^2\\
%   &\leq& c_1 2\left(\frac{C}{c_1}\gamma^{h+1} + 
%   \left[\frac{2BQC}{c_1 c_2} + \frac{C}{c_2}\right]\gamma^h \right) \\
%   &\leq& 
%   \left[2C + \frac{4BQC}{ c_2 \gamma} + \frac{c_1 2C}{c_2\gamma}\right]\gamma^{h+1} \\
%   &=& \hat{c}_2 \delta(h+1).
%  \end{eqnarray*}
%  That is every node that is $\hat{c}_2 \delta(h+1)$-suboptimal is not in the 
%  ball thus together with its descendants would never be evaluated again.
% \end{proof}
% 
% \begin{lemma}
%  If every node in $\hat{I_i}$ 
%  is evaluated or one of its descendants is evaluated and $\vx^*_{i}$ is reached
%  for $i \in \{0, 1, \cdots, h\}$,
%  then a node $\vx$ at level $h+1$ or its descendants would only be evaluated if 
%  $\vx \in \hat{I}_{h+1}$ and for at most $\frac{h+1}{\hat{k}}$ times
%  before $\vx^*_{h+1}$ is reached.
% \end{lemma}


\begin{theorem}
 If $\alpha=2$, the the cumulative regret is finite.
\end{theorem}
\begin{proof}
 By Lemma~\ref{fintime}, we have that after $\hat{n}_0$ node expansions
 any node $\vx$ that is 
 $\left[\frac{2BQC}{c_1} + C\right]\gamma^{\hat{h}_0-1}$-optimal 
 is in the ball $\calB(\vx^*, \rho)$.
 We first show that SOO-UCB would spend a finite number of evaluations
 on nodes that are
 $\left[\frac{2BQC}{c_1} + C\right]\gamma^{\hat{h}_0-1}$-suboptimal.
 Let $\hat{\epsilon} =\left[\frac{2BQC}{c_1} + C\right]\gamma^{\hat{h}_0-1}$.
 As the simple regret of SOO-UCB vanishes, within finite time we have 
 $f^+ > f^* - \frac{\hat{\epsilon}}{2}$. 
 For a $\hat{\epsilon}$-suboptimal node
 $\vx$ to be sampled $\sigma(\vx) > \frac{\hat{\epsilon}}{4B}$.
 By Lemma~\ref{levelvar}, there exist $\hat{h}_m$, such that if a node 
 $\vx_{\hat{h}_m, i}$ at
 level $\hat{h}_m$ is evaluated or one of its descendants is evaluated,
 then $\sigma(\vx) < \frac{\hat{\epsilon}}{4B}$ 
 $\forall \vx \in \calX_{\hat{h}_m, i}$. Since there is a 
 finite number of node on or below level $\hat{h}_m$, we have that 
 SOO-UCB would only spend a finite number of evaluations on 
 $\left[\frac{2BQC}{c_1} + C\right]\gamma^{\hat{h}_0-1}$-suboptimal 
 nodes. 
 
 Consider the time interval $T_h$ where
 $\vx^*_h$ is reached and $\vx^*_{h+1}$ is yet to be reached. 
 Suppose not that $\vx$ is evaluated and it is
 $\left[\frac{2BQC}{c_1} + C\right]\gamma^{h-1}$-suboptimal.
 If $\vx$ is $\left[\frac{2BQC}{c_1} + C\right]\gamma^{\hat{h}_0-1}$-suboptimal 
 nodes, then its evaluation could be attributed to the case above.
 Otherwise, let $H_0 \geq \hat{h}_0$ be the largest integer such that 
 $\vx$ is $\left[\frac{2BQC}{c_1} + C\right]\gamma^{H_0-1}$-optimal.
 Notice $h > H_0$.
 Since $c_2\|\vx - \vx^*\|^2 \leq f^* - f(\vx) 
 \leq \left[\frac{2BQC}{c_1} + C\right]\gamma^{H_0-1}$.
 we have that 
 $\vx \in \calB\left(\vx^*,  
 \sqrt{\left[\frac{2BQC}{c_1 c_2} + \frac{C}{c_2}\right]\gamma^{H_0-1}}\right)$.
 The ancestor of $\vx$ on level $H_0$ must be in 
 $\calB\left(\vx^*,  \sqrt{\frac{C}{c_1}\gamma^{H_0}} + 
 \sqrt{\left[\frac{2BQC}{c_1 c_2} + \frac{C}{c_2}\right]\gamma^{H_0-1}}\right)$
 since the radius of a cell on level $H_0$ is less than 
 $\sqrt{\frac{C}{c_1}\gamma^{H_0}}$.
 If any descendants of this ancestor of this node is evaluated, 
 then by Lemma~\ref{levelvar} $\sigma(\vx) < \frac{QC}{c_1} \gamma^{H_0}$.
 Therefore, 
 \begin{eqnarray*}
  f(\vx) + 2B\sigma(\vx) 
  &<& f^* - \left[\frac{2BQC}{c_1} + C\right]\gamma^{H_0} + 
   \frac{2BQC}{c_1} \gamma^{H_0}  \\
  &=& f^* - C\gamma^{H_0} \\
  &\leq& f^* - C\gamma^{h} \\
  &\leq& f^+.
 \end{eqnarray*}
 This contradicts the fact that $\vx$ is evaluated. 
 If we assume that every node in the ball 
 $\calB\left(\vx^*,  \sqrt{\frac{C}{c_1}\gamma^{H_0}} + 
 \sqrt{\left[\frac{2BQC}{c_1 c_2} + \frac{C}{c_2}\right]\gamma^{H_0-1}}\right)$
 is evaluated once
 we then could attribute the evaluation of $\vx$ to level $H_0$.
 We know that after 
 $K_1 h_{\max}(n) |I_{h + 1}|$ node expansions,
 the optimal node at level $h + 1$ will be expanded.
 Notice $\sqrt{n} = h_{\max} \in \mathcal{O}(h^*_n)$.
 Since we can assume that each evaluation is 
 $\left[\frac{2BQC}{c_1} + C\right] \gamma^{h-1}$-optimal,
 the total regret suffered within interval $T_h$ is of order
 $\mathcal{O}(h\gamma^h)$.
 Summing over all the time intervals would give us finite regret since
 $\sum_{i=0}^{\infty}h\gamma^h$ is finite.
 
 Finally, we show that if every node in the ball 
 $\calB\left(\vx^*,  \sqrt{\frac{C}{c_1}\gamma^{H_0}} + 
 \sqrt{\left[\frac{2BQC}{c_1 c_2} + \frac{C}{c_2}\right]\gamma^{H_0-1}}\right)$
 is evaluated once for all $H > \hat{h}_0$, 
 we again suffer only finite regret. For all nodes that
 are in the ball
 we have, 
 \begin{eqnarray*}
  f^* - f(\vx) &\leq& c_1 \left(\sqrt{\frac{C}{c_1}\gamma^{H}} + 
  \sqrt{\left[\frac{2BQC}{c_1 c_2} + \frac{C}{c_2}\right]\gamma^{H-1}}\right)^2\\
  &\leq& c_1 2\left(\frac{C}{c_1}\gamma^{H} + 
  \left[\frac{2BQC}{c_1 c_2} + \frac{C}{c_2}\right]\gamma^{H-1} \right) \\
  &\leq& 
  \left[2C + \frac{4BQC}{ c_2 \gamma} + \frac{c_1 2C}{c_2\gamma}\right]\gamma^{H} \\
  &=& \hat{c} \delta(H).
 \end{eqnarray*}
 Thus for each node in the ball at level $H$ is $\hat{c} \delta(H)$-optimal. 
 Consequently, there exist $C_{\hat{c}}$ such that the number of nodes
 in the ball is bounded by $C_{\hat{c}}\delta(H)^{-0} = C_{\hat{c}}$. 
 Summing up all the
 levels we have the total regret is less than 
 $\sum_{H = \hat{h}_0}^{\infty} C_{\hat{c}} \hat{c} \delta(H) $
 which is finite.
\end{proof}
